Human Factors in Immersive Analytics

It has been ten years since the term ''Immersive Analytics'' (IA) was coined and research interest in the topic remains strong. Researchers in this field have produced practical and conceptual knowledge concerning the use of emerging immersive spatial display and interaction technologies for sense-making tasks through a number of papers, surveys, and books. However, a lack of truly physically and psychologically ergonomic techniques, as well as standardized human-centric validation protocols for these, remains a significant barrier to wider acceptance of practical IA systems in ubiquitous applications. Building upon a series of workshops on immersive analytics at various conferences, this workshop aims to explore new approaches and establish standard practices for evaluating immersive analytics systems from a human factors perspective. We will gather immersive analytics researchers and practitioners to look closely at these human factors -- including cognitive and physical functions as well as behaviour and performance -- to see how they inform the design and deployment of immersive analytics techniques and applications and to inform future research.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/content.tex <==


\subsection{Previous Workshops}%\todo{focuses of  previous workshops can be briefly mentioned here}
This workshop will build upon previous workshops on immersive analytics, as listed below.


\begin{enumerate}
    \item ACM ISS 2016~\cite{bach2016immersive}, Immersive Analytics: Exploring Future
Interaction and Visualization
Technologies for Data Analytics. This workshop covered a wide range of topics including real-world visual analytics, collaboration, hybrid 2D and 3D, affordances for immersions, changing technologies, application areas, and platforms and toolkits. 
    %https://dl.acm.org/doi/pdf/10.1145/2992154.2996365
    
    \item IEEE VIS 2017~\cite{bach2017immersive}, Immersive Analytics: Exploring Future Visualization and Interaction
Technologies for Data Analytics. The topics of this workshop were changing technology and scenarios, hybrid 2D and 3D, affordances for immersion, collaboration, physical and tangible visualization, interaction techniques, real-world visual analytics and applications.
%http://sheelaghcarpendale.ca/innovis/uploads/Publications/Publications/carpendale2017exploring.pdf

\item ACM CHI 2019~\cite{bach2019interaction}, Interaction Design and Prototyping for Immersive Analytics. The workshop focused on prototyping and design sessions.
%http://library.usc.edu.ph/ACM/CHI2019/2exabs/W21.pdf

\item ACM CHI 2020~\cite{ens2020envisioning}, Envisioning Future Productivity for
Immersive Analytics. The workshop focused on productive user interfaces for immersive analytics (e.g., user productivity, multimodal input, collaborative analytics, users and scenarios, situated and spatial analytics, evaluation).
%https://dl.acm.org/doi/pdf/10.1145/3334480.3375145

\item ISS 2022~\cite{ISSImmersiveAnalytics2022}, Workshop on Immersive Analytics Spaces and Surfaces.  The workshop focused on exploring benefits and applications of flat versus spatial interaction affordances within immersive environments. 
%https://conf.researchr.org/track/iss-2022/immersive-analytics

\item ACM CHI 2022~\cite{ens2022immersive}, Immersive Analytics 2.0: Spatial and Embodied Sensemaking. The workshop focused on understanding immersive versus non immersive platforms for sensemaking and analytics. Topics include fundamental research questions, new evaluation methods, human-AI sensemaking, accessibile sensemaking, data physicalization, situated/embedded data visualization, and authoring immersive visualization.
%https://vtechworks.lib.vt.edu/server/api/core/bitstreams/a1d812b5-3dbc-400e-870a-4bb3450555f3/content

\end{enumerate}

While ideas derived from psychology and philosophical theories of embodied interaction were discussed in these workshops as motivation for particular design ideas, they have not yet been deeply explored.
In this workshop, we focus on understanding human factors in IA and their implications for guiding both software and hardware design of future IA systems.



\subsection{Workshop Aims}
The primary goal of this workshop is to establish a research agenda for broadening the establishments made so far in IA. We will focus on exploring the human factors that contribute to the effectiveness of IA systems in comparison to non-immersive systems. One of the core workshop outcomes will be a systematic review paper that outlines key research questions, identifies new application areas, and proposes better of evaluation methods.

Additional aims are:
\begin{itemize}
    \item Identification of fundamental human factors that contribute to the effectiveness of existing  systems in IA.
    \item Broadening our understanding of physical and cognitive benefits and limitations of IA to inform an improved expansion of IA into further application areas.
    \item To identify approaches for evaluating these human factors and techniques for addressing their limitations.
\end{itemize}
%This workshop aims at sparking discussion around cognitive and sensory aspects of immersive analytics among researchers and practitioners. The cognitive aspects may include cognitive psychology concepts stated in \citet{goldstein2015cognitive}: perception, attention, memory, knowledge, visual imagery, language, problem solving, reasoning and decision making. The sensory-motor aspects may include ...

%Cognition is a broad topic that can be  looked at from multiple perspectives. 

%Cognitive science is a branch of science that investigates how cognition works by incorporating multiple disciplines (e.g., psychology, philosophy, artificial intelligence, neuroscience anthropology, and linguistics)~\cite{bermudez2014cognitive}. 

%We focus on a simple step that looks at cognitive psychology. 
% The objectives of this workshop are: 
% \begin{enumerate}
%     \item to spark the discussion among experts (forming potential collaborations) 
%     \item to start early work on how to conceptualise cognition and SAI (forming future agenda)
% \end{enumerate}

\subsection{Perspectives of Interest}
\label{sec:challenges}
This workshop will explore a series of research questions focused on cognitive and physical aspects, and how to consider these aspects in IA. These include looking at cognitive and physical aspects independently, the integration between the two aspects, and how to adapt the user interface considering these aspects to improve system efficiency. These questions will focus on a group of themes as below:

\noindent\textbf{Fundamental Cognitive Factors In System Design} -- 
%Designs in previous immersive analytics system 
Understanding the roles of cognition and perception, including attention, memory, knowledge, visual imagery, language, problem solving, reasoning and decision making, and relevant scenarios is crucial for improving IA interface design. 

    %\item How do the relationship between one's cognitive aspects, immersive analytics tools, and the data differ from traditional desktop analytics?
    
%\begin{enumerate}
   % \item In what scenarios would perception, attention, memory, knowledge, visual imagery, language, problem solving, reasoning and decision making play an important role in immersive analytics?
  %  \item How do the relationship between one's cognitive aspects, immersive analytics tools, and the data differ from traditional desktop analytics?
    % included overarching research questions below [from the perspective of mental models]:
    %\item How do end-users' mental models of immersive analytics tools influence their data comprehension and decision-making processes, both individually and collaboratively?
    %\item What cognitive challenges and barriers do novice users encounter while interacting with data in immersive analytics environments- How do these challenges differ from those faced in non-immersive, traditional analytics contexts?
    %\item What strategies or interventions can effectively mitigate the cognitive and conceptual challenges users experience in immersive analytics environments?
    % \begin{enumerate}
    %     \item How can these solutions enhance users' overall data interpretation, insight generation, and decision-making processes?
    % \end{enumerate}
%\end{enumerate}

\noindent\textbf{Fundamental Physical Factors In System Design} -- Using body movements as input to interact with IA systems is widely adopted in literature. However, little discussion has yet been made about how these input modalities support analytical tasks. A wide variety of physical factors require further consideration including human biomechanical limitations on movement such as maximum speed, accuracy and fatigue over time.

\noindent\textbf{Synergistic Effect Between Cognitive And Physical Factors} -- Novel gestures were proposed to manipulate diverse types of data and information. We will discuss how users' mental models of such techniques influence their comprehension and decision-making processes in analytic tasks with consideration of theories of distributed cognition and kinesthetic memory effects.

\noindent\textbf{New Evaluation Methods And Research Methods} -- Previous system evaluation relies on performance metrics, such as, completion time and accuracy, and post-study subjective preference. New research agendas are needed to establish a better practice of system evaluation with the recently developed techniques in measuring the cognitive and physical cost during interaction time. 

\noindent\textbf{Novel Interaction Technique} -- A wide range of prior work has been done to reduce the cognitive and physical cost during interaction. However, questions about how these solutions can enhance users' overall data interpretation, insight generation, and decision-making processes and in what type of analytic tasks remain unsolved.

\noindent\textbf{Adaptive User Interfaces} -- Online optimization is an established technique to adapt interfaces to consider human factors such as cognitive load and visibility \cite{lindlbauer2019online}.  Recent toolkits facilitate the usage of optimization and abstract the formulation of  such mathematical problems through adaptation objectives \cite{belo2022auit}. Novel formulations of cognitive and physical factors as adaptation objectives are a requirement to make optimization with respect to these factors accessible to creators. Additionally, IA applications have unique requirements that must be identified and addressed to ensure effective adaptations.

\section{ORGANIZERS}

The group of organizers consist of academics and representatives from industry with with diverse backgrounds (i.e., immersive analytics, general XR interaction, empathic computing, XR, VR, AR, and affective computing). These include organizers from previous Immersive Analytics workshops (Satriadi, Liu,
Dwyer). The organizing team consists of a diverse group of senior, mid-career, and early-career academics, as well as students with expertise in fatigue modeling in XR, accessible and inclusive VR, and mental models in AR interactions. They are from 5 different countries and 6 different institutions.

%Organisers do not have to be experts in the areas. 
\noindent\textbf{Yi Li} is a Ph.D. student in the Embodied Visualisation research group at Monash University, Australia. Her main research direction focuses on mitigating physical fatigue in adaptive XR interaction. She recently published a comprehensive shoulder fatigue model to assist future gestural interaction design~\cite{li2024nicer}.

\noindent\textbf{Kadek Satriadi} is a Lecturer at Monash University Australia in the Embodied Visualisation research group. His research revolves around IA for geospatial data, situated scenarios, storytelling, and physicalizations. He was a co-organiser of the  IA workshops at ISS 2022 and CHI 2022, and a technology co-chair at IEEE VIS 2023.  

\noindent\textbf{Jiazhou `Joe' Liu} is a Postdoctoral Fellow working at the Embodied Visualisation research group at Monash University, Australia. He co-organised the ``Immersive Analytics 2.0'' workshop at CHI 2022. His research focus is on immersive visualisation view management, specialising in spatial cognition and skills. His recent research explores AI in IA, with applications in medical and construction domains.

\noindent\textbf{Anjali Khurana} is a Ph.D. student at Simon Fraser University (SFU), Burnaby, Canada. Her research interest lies in understanding users’ mental models when employing novel interaction paradigms, such as gestural interactions with AR and prompt-based interactions with LLMs for their software tasks, and further inventing onboarding and assistance techniques for novice users of AR and LLMs. her work has been published at top HCI venues including, ACM IUI 2024, and Proc. ACM Interact. Mob. Wearable Ubiquitous Technol. (IMWUT 2023).

\noindent\textbf{Zhiqing Wu} is a Ph.D. student at The Hong Kong University of Science and Technology (Guangzhou), China. Her research interest lies on making VR interaction more inclusive and accessible. Her work on understanding VR interaction for older adults has been recently published in CHI 2024.

\noindent\textbf{João Belo} is a Postdoctoral Fellow at the Computational Interaction Group at Saarland University. His research focuses on Computational Interaction and Extended Reality, exploring optimization and machine learning methods to improve interaction in 2D and 3D user interfaces. Recent work proposes methods to facilitate the consideration of human factors, such as ergonomics, in adaptive user interfaces and how to optimize these in real time.

\noindent\textbf{Arindam Dey} is a leading Research Scientist in the Reality Lab at Meta working on mitigating visual discomfort in VR and MR with machine learning and physiological computing. Previously, he was a lecturer at the University of Queensland where he founded and directed the Empathetic XR and Pervasive Computing Lab. 

\noindent\textbf{Benjamin Tag} is a Senior Lecturer at UNSW Sydney, specializing in Human-Computer Interaction, Affective Computing, and Human-AI Interaction. His research focuses on technologies for assessing mental~\cite{Tag2019} and physical states~\cite{li2024nicer} in real-world and virtual environments, with an emphasis on human emotion, cognitive psychology, and context-aware computing. 

\noindent\textbf{Tim Dwyer} is Professor of Computer Science and Director of the Embodied Visualisation Research Group at Monash University, Australia. He has been exploring topics in immersive data visualisation for 24 years and co-authored the earliest papers establishing the topic of IA (e.g. \cite{7314296}). He edited the original book \cite{marriott2018immersive}, after co-organizing the first Dagstuhl Seminar on IA.


\section{PRE-WORKSHOP PLANS}
To recruit participants, we will advertise a call for participation within the standard CHI mailing list, as well as the organizers networks and on social media. We will launch our website (\url{https://sites.google.com/monash.edu/iahf-workshop}) to communicate the Call For Participation and provide participants with general instructions, such as the background and motivation, pre-workshop activities, submission deadlines, and contact information of the organisers. In the later stage, workshop submissions (e.g., written statements and/or videos) may also be made publicly available on the website upon acceptance of the workshop and consent from the participants. 

\subsection{Workshop Structure}
The workshop will be run \textbf{in-person} to ensure a high quality of engagement for participants. We aim to attract the in-person workshop attendance limit of 35. If we receive more than 35 applications then we will select participants based on the quality and suitability of their submissions using a light-weight peer-review process, selecting reviewers from the wider community as necessary. We will publish the workshop proceedings on CEUR-WS.org\url{https://ceur-ws.org/}. Our workshop will focus on generating ideas through discussion, hence we do not expect to have paper presentations. We rather aim to follow up this workshop with a publication plan and future workshops (see section \ref{post}). We will accommodate accessibility for special requirements as requested by participants the registration process.

\section{ASYNCHRONOUS ENGAGEMENT}
We will share a google drive folder containing all related activities prior to the workshop. These include workshop brief, schedule, and code of conduct. Prior to the workshop, participants will be asked to prepare a written statement 1 to 4 pages in length (excluding references) and/or a maximum 3-minute video response addressing our proposed research topics and challenges (see~\autoref{sec:challenges} for more details). These may include examples from their own work or other research related to their expertise. The submitted responses will be stored in a secured Google Drive folder and reviewed by the workshop organizers. This activity will be conducted asynchronously. 

\section{MAIN WORKSHOP ACTIVITIES}
%Explain the activities you plan to do during the workshop (e.g., keynote, workshop paper presentations).
The main workshop activities will focus on lightning talks, live demonstrations, and group discussions on proposed topics. The schedule of the activities in \autoref{tab:schedule} is proposed based on the format of previous CHI workshops (i.e., two 80-minute sessions for a \textbf{half-day} workshop). 

\input{paper/schedule-table}

%\textbf{Welcome and Introduction (5 minutes)} --- At the beginning of the workshop, organisers will kick off and introduce themselves, as well as the motivation for the workshop. They will provide an overview of the scheduled activities.
% 5 mins

%\textbf{Keynote (15 minutes)} --- We will invite one domain expert to provide a motivational speech about the topic. The keynote will establish the basic tone and tenor for this workshop and may come with engaging stories and example research about the proposed challenges. 


%\textbf{Lightning Talks (30 minutes)} --- Before the workshop, all participants will be asked whether or not they are willing to give a lightning talk about the material they prepared in the pre-workshop submissions. During the workshop, those participants will take turns giving an introduction and brief overview of the response addressing the listed topic/challenges. 
%The duration of this session will depend on the number of participants and their willingness.

%\textbf{Group Discussion (30 minutes)} --- In this first set of group discussions, participants will divide into groups (of around 5-8), each with a focus on one of the key human factors under consideration: Cognitive, Perceptual, Biomechanical, Sensory-Motor, collaboration. 


%\textbf{CHI conference official break (40 mins)}

%\textbf{Video Showcase and Live Demonstrations (30 minutes)} --- A break is expected to be scheduled after the first group discussion. During the break, participants who would like to showcase their work relevant to the workshop topics will set up the videos and demos in the allocated space. The workshop organisers will also prepare for a few demos during the break. 
%After the break, other participants will move around in the workshop room and chat with those who have a video or a demo. 

%\textbf{Group Discussion: Topic 2 (40 minutes)} --- The second discussion session will focus on ...

%\textbf{Closing and Summary (10 minutes)} --- The closing session of the workshop will centre on reviewing the workshop's activities and outlining future steps. Organisers will start by summarising the events, covering the topics introduced during pre-workshop activities, and highlighting the key takeaways from the two group discussions. A final group discussion will then be held to identify action points for advancing and executing the roadmap created during the workshop. This discussion will also explore potential follow-up publications and plans for future workshops or events to strengthen the community. 

\section{POST-WORKSHOP PLANS}
\label{post}

%State your plans for follow-up and creation of tangible outcomes (e.g., poster presentation, publication of a workshop report, plans for a special issue of a journal).
The workshop will be followed by a variety of activities:
\begin{enumerate}
    \item \textbf{Position paper} -- following the pattern of past workshops we aim to publish a peer-review position paper including a comprehensive report on the state of understanding of human factors in IA and an agenda for future research.
    \item \textbf{Working group papers} -- we are confident that the focused discussion groups will spawn new networks leading to independent research and eventually co-authorship on these specific sub-topics.
    \item \textbf{Future workshops} -- there is scope for future workshops more specialized to each of the subtopics within human factors in IA as well as application to future effective IA system design and technological as well as societal readiness.
\end{enumerate}

\section{CALL FOR PARTICIPATION}
Join us for an exploration of topics on ``Human Factors in Immersive Analytics'' workshop, to be held at ACM CHI 2025. This workshop will focus on the cognitive, perceptual, biomechanical, sensory-motor, and collaborative aspects of Immersive Analytics and how these factors influence sensemaking and data comprehension. While immersive technologies have shown potential in analytics, many open research questions remain concerning the human factors that shape the effective use of immersive analytics applications. 
We encourage researchers, practitioners, and designers to submit research papers, early-stage work, or conceptual ideas, ranging from 1 to 4 pages (excluding references), in the standard CHI submission format. 
Each paper will be reviewed by the organizers to ensure quality and relevance. 
All accepted papers will be compiled and made available to all participants ahead of the workshop, facilitating pre-event engagement and discussion. A selection of papers will be published after the workshop on the CEUR-WS.org website, where authors can choose to opt in for it. At least one author of each accepted submission must register and attend the workshop. The program will consist of a keynote, live demonstrations, and group discussions, focusing on topics such as fundamental cognitive factors in system design, fundamental physical factors in system design, the synergistic effect between cognitive and physical factors, new evaluation and research methods, novel interaction techniques, and adaptive user interfaces. More details about the workshop can be found at \url{https://sites.google.com/monash.edu/iahf-workshop}. 
    
    % \item \textbf{Empirical studies} on the cognitive roles and barriers in immersive analytics
    % \item Examination of how \textbf{cognitive processes and interactions} with data in immersive analytics tools differ from those in traditional desktop-based analytics systems
    % \item \textbf{Design processes and strategies} for supporting data interpretation and decision-making in immersive analytics 
    % \item Research into how users’\textbf{ mental models} influence their interaction with immersive analytic tools and vice versa
    % \item Exploration of scenarios highlight the \textbf{importance of cognitive processes} such as perception, attention, memory, visual imagery, language, problem solving, reasoning, and decision-making in immersive analytics environments
    % \item \textbf{Novel interaction techniques and interventions} for enhancing data comprehension and overcoming cognitive challenges in immersive analytics


%\subsection{Submission Guidelines}
%We invite submissions of papers, ranging from 1 to 4 pages in length (excluding references), that explore innovative ideas, including both early-stage and ongoing research, or work that has been recently completed. Each paper will undergo a peer-review process to ensure quality and relevance, although they will not be published in a formal proceedings. All accepted papers will be compiled and made available to all participants ahead of the workshop, facilitating pre-event engagement and discussion.

\section{Important Dates}
%Paper Submission: Thursday, February 13, 2025 Anywhere on Earth (AoE) time zone
%Author Notification: Friday, March 14, 2025

\begin{table}[H]
\begin{tabular}{ll}
\multicolumn{1}{l}{\textbf{Activity}} & \multicolumn{1}{l}{\textbf{Date}} \\ \hline
Website and CFP launches                & December 16, 2024                  \\
EOI deadline                            & February 1, 2025                   \\
Acceptance notification                 & March 1, 2025                      \\
Asynchronous material shared            & April 2025                         \\
Workshop at CHI 2025                    & May 2025                          
\end{tabular}
\caption{Workshop important dates}
\end{table}

% ISS template and modify w.r.t timeline for CHI
%Provide a 250-word Call for Participation that will be posted on the conference site to recruit participants for your workshop. This should appear at the end of your workshop proposal and should include the following:
%The format (including adequacy to in-person or hybrid format) and goals of the workshop
%The participant selection criteria
%Requirements for participants’ submissions (e.g., topics to address, page length, format)
%Where should these papers be submitted
%How accepted workshop papers will be published
%The requirement that at least one author of each accepted submission must attend the workshop and that all participants must register for both the workshop and for at least one day of the conference.
%A link to the workshop website.




==> sections/intro.tex <==
%\section{INTRODUCTION AND MOTIVATION}
%\todo{All, feel free to improve this section}
%Provide a strong rationale for the workshop, describe the issues to be addressed, and state concrete objectives.

The field of Immersive Analytics (IA) operates under the idea that work environments that bring data into the space around the user (or \textit{users} in collaborative contexts) promote effective and engaging sensemaking activities~\cite{dwyer2018immersive}. Steady development and release of new devices---such as Apple's Vision Pro, Meta headsets (e.g., Quest 3 and 3s) and glasses (e.g., Orion glasses), Pico's Pico 4 Ultra, Varjo's XR 4, and more---demonstrates a positive trend for the future of IA, with technical barriers to adoption gradually dropping away. Yet, our understanding of the human aspects of IA---i.e., the capabilities of humans to operate with information presented in immersive environments---lags behind the rapid development of the supporting hardware. 

Human factors---including cognitive and physical functions, behavior, and performance---in IA applications still pose open research questions. So far, we have witnessed significant milestones in the field, including---but not limited to---a textbook~\cite{marriott2018immersive}, surveys of IA and situated analytics (IA employing Augmented Reality to situate information in a real-world evironment)~\cite{fonnet2019survey, zhao2022metaverse, kraus2022immersive, saffo2023unraveling, Lee:2023:DesignPatterns, Satriadi:2023:ProxSituated, bressa2021s}, lists of challenges and agendas\cite{skarbez2019immersive, ens2021grand}, and results on graphical perception\cite{whitlock2020graphical}. Nevertheless, we have yet to start exploring the theoretical aspects of IA, as shown by a recent review~\cite{saffo2023unraveling} and mentioned in a grand challenge paper~\cite{ens2021grand}. It is apparent that the ``what technique works'' topics have been seen more often than ``why a technique works'', especially when we reflect on the role of cognitive and physical factors of the user. Considering the growing interest in measuring IA techniques beyond performance, such as memory \cite{liu2022effects, liu:2024:LandmarkSpatialMemory, han2023evaluating, hurter2024memory}, learning~\cite{khurana2024just}, physical reach and strength~\cite{evangelista2021xrgonomics, wu2024toward, li2023revisiting}, and physical fatigue~\cite{dai2024precise, li2024nicer}, it is the right time to define relevant human factors in IA, and how we should go about measuring them.  

This workshop aims to contribute to this by defining a roadmap for new directions in understanding the human characteristics when interacting with immersive content to optimize the design of IA systems. Through a combination of synchronous and asynchronous sessions, along with in-person discussion, we will gather researchers from diverse backgrounds and expertise. Participants will come from IA and related fields, including interaction design, data visualization, VR, AR, biomechanics, embodied cognition, and more, offering a broad array of viewpoints.

By fostering interdisciplinary collaboration of experts, this workshop will pave the way for defining key human factors and establish robust methodologies for measuring and optimizing user interaction with immersive analytics systems.


==> sections/teaser.tex <==
\teaser{
  \centering
  \includegraphics[width=\linewidth]{figures/teaser.pdf}
  \caption{Understanding human factors in immersive analytics can pave the way for better interface design. This workshop will look closely at mental (illustrated as the red parts of the users in the left figure) and physical aspects (red parts in the right figure) involved in immersive analytics applications, including how to better measure related factors.}
  %\Description{Immersive analytics scenarios}
  \label{fig:teaser}
}

